Behavioural Reports of Multi-Stage Malware

The extensive damage caused by malware requires anti-malware systems to be constantly improved to prevent new threats. The current trend in malware detection is to employ machine learning models to aid in the classification process. We propose a new dataset with the objective of improving current anti-malware systems. The focus of this dataset is to improve host based intrusion detection systems by providing API call sequences for thousands of malware samples executed in Windows 10 virtual machines. A tutorial on how to create and expand this dataset is provided along with a benchmark demonstrating how to use this dataset to classify malware. The data contains long sequences of API calls for each sample, and in order to create models that can be deployed in resource constrained devices, three feature selection methods were tested. The principal innovation, however, lies in the multi-label classification system in which one sequence of APIs can be tagged with multiple labels describing its malicious behaviours.

==> Tables-old/acc-f1-table.tex <==
\begin{tabular}{lllllll}
\hline
\multirow{2}{*}{Models} & \multicolumn{2}{c}{First} & \multicolumn{2}{c}{Last} & \multicolumn{2}{c}{Random} \\
\cline{2-7}
    & Acc & F1 & Acc & F1 & Acc & F1 \\
\hline
SEM     & 0.443987 & 0.682041 & 0.407643 & 0.655089 & 0.414762 & 0.655801 \\
MLP     & 0.510303 & 0.711403 & 0.467216 & 0.690908 & 0.426002 & 0.662383 \\
LSTM    & 0.405395 & 0.652829 & 0.458973 & 0.683803 & 0.408018 & 0.65399  \\
GRU     & 0.530161 & 0.724454 & 0.479206 & 0.68739  & 0.464219 & 0.680854 \\
BiLSTM  & 0.481828 & 0.705945 & 0.467216 & 0.680692 & 0.450356 & 0.67135  \\
BiGRU   & 0.529412 & 0.71485  & 0.483327 & 0.696503 & 0.472462 & 0.684251 \\
\hline
\end{tabular}

==> Tables-old/binary-cross-entropy-table.tex <==
\begin{tabular}{lllllll}
\hline
\multirow{2}{*}{Models} & \multicolumn{2}{c}{First} & \multicolumn{2}{c}{Last} & \multicolumn{2}{c}{Random} \\
\cline{2-7}
    & Loss & BCE & Loss & BCE & Loss & BCE \\
\hline
SEM     & 0.17767  & 0.837767 & 0.184881 & 0.811165 & 0.190606 & 0.817909 \\ 
MLP     & 0.160002 & 0.835519 & 0.172008 & 0.831772 & 0.183933 & 0.827651 \\ 
LSTM    & 0.187377 & 0.816785 & 0.180346 & 0.825403 & 0.199172 & 0.811915 \\ 
GRU     & 0.148822 & 0.853128 & 0.17141  & 0.822031 & 0.168487 & 0.835519 \\ 
BiLSTM  & 0.164752 & 0.811915 & 0.174822 & 0.837018 & 0.186019 & 0.827276 \\ 
BiGRU   & 0.149932 & 0.813788 & 0.168554 & 0.838142 & 0.171527 & 0.844511 \\ 
\hline
\end{tabular}

==> Tables-old/data-distribution.tex <==
\begin{tabular}{lrrr}
    \hline
    Name        & Train & Test & Total \\
    \hline
    benign      & 66    & 35   & 101 \\
    malware     & 905   & 426  & 1331 \\
    trojan      & 4369  & 2167 & 6536 \\
    banker      & 1089  & 521  & 1610 \\
    pua         & 544   & 278  & 822 \\
    downloader  & 452   & 266  & 718 \\
    adware      & 642   & 332  & 974 \\
    dropper     & 236   & 108  & 344 \\
    spyware     & 122   & 65   & 187 \\
    virus       & 208   & 118  & 326 \\
    miner       & 69    & 33   & 102 \\
    ransomware  & 177   & 87   & 264 \\
    worm        & 155   & 82   & 237 \\
    hacktool    & 87    & 36   & 123 \\
    fakeav      & 4     & 6    & 10 \\
    \hline
\end{tabular}

==> Tables-old/first-acc-f1-table.tex <==
\begin{tabular}{lrr}
\hline
 Models   &   Accuracy &   F1-score \\
\hline
 SEM      &   0.443987 &   0.682041 \\
 MLP      &   0.510303 &   0.711403 \\
 LSTM     &   0.405395 &   0.652829 \\
 GRU      &   0.530161 &   0.724454 \\
 BiLSTM   &   0.481828 &   0.705945 \\
 BiGRU    &   0.529412 &   0.71485  \\
\hline
\end{tabular}

==> Tables-old/first-eval-table.tex <==
\begin{tabular}{lrr}
\hline
 Model   &     loss &   accuracy \\
\hline
 SEM     & 0.17767  &   0.837767 \\
 MLP     & 0.160002 &   0.835519 \\
 LSTM    & 0.187377 &   0.816785 \\
 GRU     & 0.148822 &   0.853128 \\
 BiLSTM  & 0.164752 &   0.811915 \\
 BiGRU   & 0.149932 &   0.813788 \\
\hline
\end{tabular}

==> Tables-old/first-f1-table.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\hline
 Model   &   benign &   malware &   trojan &   banker &       pua &   downloader &   adware &   dropper &   spyware &    virus &   miner &   ransomware &     worm &   hacktool &   fakeav \\
\hline
 SEM     & 0        & 0.399329  & 0.909052 & 0.824131 & 0         &     0        & 0.011976 &         0 &         0 & 0        &       0 &    0.242991  & 0        &          0 &        0 \\
 MLP     & 0        & 0.385009  & 0.908346 & 0.874031 & 0.0689655 &     0        & 0.543568 &         0 &         0 & 0.613757 &       0 &    0.562963  & 0.728477 &          0 &        0 \\
 LSTM    & 0        & 0.0318907 & 0.898539 & 0.834646 & 0         &     0        & 0        &         0 &         0 & 0.222222 &       0 &    0         & 0.091954 &          0 &        0 \\
 GRU     & 0        & 0.452381  & 0.916044 & 0.900675 & 0.224299  &     0.131944 & 0.664273 &         0 &         0 & 0.586207 &       0 &    0.549296  & 0.712121 &          0 &        0 \\
 BiLSTM  & 0        & 0.343396  & 0.912273 & 0.866    & 0         &     0        & 0.57931  &         0 &         0 & 0.467066 &       0 &    0.0224719 & 0.566929 &          0 &        0 \\
 BiGRU   & 0.166667 & 0.412969  & 0.908526 & 0.896016 & 0.237082  &     0.196203 & 0.678141 &         0 &         0 & 0.601093 &       0 &    0.594203  & 0.765957 &          0 &        0 \\
\hline
\end{tabular}

==> Tables-old/last-acc-f1-table.tex <==
\begin{tabular}{lrr}
\hline
 Models   &   Accuracy &   F1-score \\
\hline
 SEM      &   0.407643 &   0.655089 \\
 MLP      &   0.467216 &   0.690908 \\
 LSTM     &   0.458973 &   0.683803 \\
 GRU      &   0.479206 &   0.68739  \\
 BiLSTM   &   0.467216 &   0.680692 \\
 BiGRU    &   0.483327 &   0.696503 \\
\hline
\end{tabular}

==> Tables-old/last-eval-table.tex <==
\begin{tabular}{lrr}
\hline
 Model   &     loss &   accuracy \\
\hline
 SEM     & 0.184881 &   0.811165 \\
 MLP     & 0.172008 &   0.831772 \\
 LSTM    & 0.180346 &   0.825403 \\
 GRU     & 0.17141  &   0.822031 \\
 BiLSTM  & 0.174822 &   0.837018 \\
 BiGRU   & 0.168554 &   0.838142 \\
\hline
\end{tabular}

==> Tables-old/last-f1-table.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\hline
 Model   &   benign &   malware &   trojan &   banker &   pua &   downloader &   adware &   dropper &   spyware &    virus &   miner &   ransomware &      worm &   hacktool &   fakeav \\
\hline
 SEM     &        0 & 0.0227273 & 0.895491 & 0.864173 &     0 &    0         & 0        &         0 &         0 & 0.28777  &       0 &    0         & 0.0705882 &          0 &        0 \\
 MLP     &        0 & 0.401316  & 0.907472 & 0.870334 &     0 &    0         & 0.117318 &         0 &         0 & 0.581633 &       0 &    0         & 0.745098  &          0 &        0 \\
 LSTM    &        0 & 0.343537  & 0.901165 & 0.868447 &     0 &    0         & 0.220657 &         0 &         0 & 0.542553 &       0 &    0         & 0.675497  &          0 &        0 \\
 GRU     &        0 & 0.384738  & 0.901849 & 0.877368 &     0 &    0         & 0.388664 &         0 &         0 & 0.548387 &       0 &    0.0227273 & 0.693878  &          0 &        0 \\
 BiLSTM  &        0 & 0.333932  & 0.902778 & 0.876494 &     0 &    0         & 0.327801 &         0 &         0 & 0.551351 &       0 &    0         & 0.693878  &          0 &        0 \\
 BiGRU   &        0 & 0.348624  & 0.909052 & 0.883768 &     0 &    0.0649819 & 0.386813 &         0 &         0 & 0.557377 &       0 &    0.0652174 & 0.703448  &          0 &        0 \\
\hline
\end{tabular}

==> Tables-old/random-acc-f1-table.tex <==
\begin{tabular}{lrr}
\hline
 Models   &   Accuracy &   F1-score \\
\hline
 SEM      &   0.414762 &   0.655801 \\
 MLP      &   0.426002 &   0.662383 \\
 LSTM     &   0.408018 &   0.65399  \\
 GRU      &   0.464219 &   0.680854 \\
 BiLSTM   &   0.450356 &   0.67135  \\
 BiGRU    &   0.472462 &   0.684251 \\
\hline
\end{tabular}

==> Tables-old/random-eval-table.tex <==
\begin{tabular}{lrr}
\hline
 Model   &     loss &   accuracy \\
\hline
 SEM     & 0.190606 &   0.817909 \\
 MLP     & 0.183933 &   0.827651 \\
 LSTM    & 0.199172 &   0.811915 \\
 GRU     & 0.168487 &   0.835519 \\
 BiLSTM  & 0.186019 &   0.827276 \\
 BiGRU   & 0.171527 &   0.844511 \\
\hline
\end{tabular}

==> Tables-old/random-f1-table.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\hline
 Model   &   benign &   malware &   trojan &   banker &       pua &   downloader &   adware &   dropper &   spyware &    virus &   miner &   ransomware &     worm &   hacktool &   fakeav \\
\hline
 SEM     &        0 &  0.200803 & 0.897093 & 0.829171 & 0         &            0 & 0        &         0 &         0 & 0        &       0 &            0 & 0        &          0 &        0 \\
 MLP     &        0 &  0.305455 & 0.900625 & 0.832347 & 0         &            0 & 0        &         0 &         0 & 0        &       0 &            0 & 0        &          0 &        0 \\
 LSTM    &        0 &  0        & 0.896195 & 0.854086 & 0         &            0 & 0        &         0 &         0 & 0        &       0 &            0 & 0        &          0 &        0 \\
 GRU     &        0 &  0.380137 & 0.904573 & 0.870352 & 0         &            0 & 0.433198 &         0 &         0 & 0.45614  &       0 &            0 & 0.385321 &          0 &        0 \\
 BiLSTM  &        0 &  0.342762 & 0.899913 & 0.856299 & 0         &            0 & 0.276029 &         0 &         0 & 0        &       0 &            0 & 0        &          0 &        0 \\
 BiGRU   &        0 &  0.377816 & 0.907053 & 0.879433 & 0.0673401 &            0 & 0.382222 &         0 &         0 & 0.450262 &       0 &            0 & 0.556391 &          0 &        0 \\
\hline
\end{tabular}

==> Tables/eval-slices.tex <==
\begin{tabular}{lllllllllllll}
\hline
\multirow{2}{*}{Models} & \multicolumn{4}{c}{First} & \multicolumn{4}{c}{Last} & \multicolumn{4}{c}{Random} \\
\cline{2-13}
    & loss &   binary accuracy &   precision &   recall & loss &   binary accuracy &   precision &   recall & loss &   binary accuracy &   precision &   recall \\
\hline
SEM     & 0.177671 & 0.940202 & 0.845344 & 0.58136  & 0.184881 & 0.93768  & 0.824788 & 0.575    & 0.190606 & 0.937555 & 0.832473 & 0.56557 \\ 
MLP     & 0.159986 & 0.946822 & 0.847783 & 0.649781 & 0.172009 & 0.943225 & 0.847463 & 0.611623 & 0.183933 & 0.938579 & 0.840078 & 0.569079\\ 
LSTM    & 0.181599 & 0.938429 & 0.823003 & 0.585307 & 0.180586 & 0.941851 & 0.850063 & 0.594298 & 0.198424 & 0.93703  & 0.82171  & 0.571053\\ 
GRU     & 0.148572 & 0.951218 & 0.870839 & 0.671272 & 0.17141  & 0.94255  & 0.83651  & 0.616009 & 0.178398 & 0.942126 & 0.860727 & 0.586842\\ 
BiLSTM  & 0.16571  & 0.945348 & 0.858092 & 0.623246 & 0.171951 & 0.943774 & 0.843908 & 0.621272 & 0.189791 & 0.938479 & 0.827145 & 0.58136 \\ 
BiGRU   & 0.149645 & 0.94912  & 0.856255 & 0.664912 & 0.168341 & 0.944823 & 0.849955 & 0.626096 & 0.170241 & 0.942875 & 0.844917 & 0.610526\\ 
\hline
\end{tabular}

==> Tables/first-acc-f1-table.tex <==
\begin{tabular}{lrr}
\hline
 Models   &   Accuracy &   F1-score \\
\hline
 SEM      &   0.443987 &   0.682041 \\
 MLP      &   0.510303 &   0.711403 \\
 LSTM     &   0.416261 &   0.656551 \\
 GRU      &   0.531285 &   0.722218 \\
 BiLSTM   &   0.487823 &   0.684139 \\
 BiGRU    &   0.52529  &   0.707119 \\
\hline
\end{tabular}

==> Tables/first-eval-table.tex <==
\begin{tabular}{lllll}
\hline
 Model   &     loss &   binary accuracy &   precision &   recall \\
\hline
 SEM     & 0.177671 &          0.940202 &    0.845344 & 0.58136  \\
 MLP     & 0.159986 &          0.946822 &    0.847783 & 0.649781 \\
 LSTM    & 0.181599 &          0.938429 &    0.823003 & 0.585307 \\
 GRU     & 0.148572 &          0.951218 &    0.870839 & 0.671272 \\
 BiLSTM  & 0.16571  &          0.945348 &    0.858092 & 0.623246 \\
 BiGRU   & 0.149645 &          0.94912  &    0.856255 & 0.664912 \\
\hline
\end{tabular}

==> Tables/last-acc-f1-table.tex <==
\begin{tabular}{lrr}
\hline
 Models   &   Accuracy &   F1-score \\
\hline
 SEM      &   0.407643 &   0.655089 \\
 MLP      &   0.467216 &   0.690908 \\
 LSTM     &   0.448483 &   0.674023 \\
 GRU      &   0.479206 &   0.68739  \\
 BiLSTM   &   0.48033  &   0.695775 \\
 BiGRU    &   0.483327 &   0.698252 \\
\hline
\end{tabular}

==> Tables/last-eval-table.tex <==
\begin{tabular}{lllll}
\hline
 Model   &     loss &   binary accuracy &   precision &   recall \\
\hline
 SEM     & 0.184881 &          0.93768  &    0.824788 & 0.575    \\
 MLP     & 0.172009 &          0.943225 &    0.847463 & 0.611623 \\
 LSTM    & 0.180586 &          0.941851 &    0.850063 & 0.594298 \\
 GRU     & 0.17141  &          0.94255  &    0.83651  & 0.616009 \\
 BiLSTM  & 0.171951 &          0.943774 &    0.843908 & 0.621272 \\
 BiGRU   & 0.168341 &          0.944823 &    0.849955 & 0.626096 \\
\hline
\end{tabular}

==> Tables/random-acc-f1-table.tex <==
\begin{tabular}{lrr}
\hline
 Models   &   Accuracy &   F1-score \\
\hline
 SEM      &   0.414762 &   0.655801 \\
 MLP      &   0.426002 &   0.662383 \\
 LSTM     &   0.408018 &   0.654128 \\
 GRU      &   0.452229 &   0.673273 \\
 BiLSTM   &   0.441738 &   0.665418 \\
 BiGRU    &   0.467216 &   0.6852   \\
\hline
\end{tabular}

==> Tables/random-eval-table.tex <==
\begin{tabular}{lllll}
\hline
 Model   &     loss &   binary accuracy &   precision &   recall \\
\hline
 SEM     & 0.190606 &          0.937555 &    0.832473 & 0.56557  \\
 MLP     & 0.183933 &          0.938579 &    0.840078 & 0.569079 \\
 LSTM    & 0.198424 &          0.93703  &    0.82171  & 0.571053 \\
 GRU     & 0.178398 &          0.942126 &    0.860727 & 0.586842 \\
 BiLSTM  & 0.189791 &          0.938479 &    0.827145 & 0.58136  \\
 BiGRU   & 0.170241 &          0.942875 &    0.844917 & 0.610526 \\
\hline
\end{tabular}
